TLDR: Extreme Summarization of Scientific Documents

We introduce TLDR generation, a new form of extreme summarization, for scientific papers. TLDR generation involves high source compression and requires expert background knowledge and understanding of complex domain-specific language. To facilitate study on this task, we introduce SciTLDR, a new multi-target dataset of 5.4K TLDRs over 3.2K papers. SciTLDR contains both author-written and expert-derived TLDRs, where the latter are collected using a novel annotation protocol that produces high-quality summaries while minimizing annotation burden. We propose CATTS, a simple yet effective learning strategy for generating TLDRs that exploits titles as an auxiliary training signal. CATTS improves upon strong baselines under both automated metrics and human evaluations. Data and code are publicly available at https://github.com/allenai/scitldr.

==> backup-04-baselines.tex <==
\section{Baselines}\label{sec:baselines}
% Previous studies have found that the most salient information in a paper for writing a summary is often found in the abstract, introduction, and conclusion \insertcite. Therefore, we hypothesize that a model should be able to learn to generate \tldrs using only these sections. This hypothesis is further supported by our oracle analysis, which shows that the performance gains from including the introduction and conclusion in addition to the abstract are greater than including the full text from AIC. \isabel{some editing needed here}
% However, another reasonable input space is to constrain the input to only the abstract of the paper and generate \tldr from that. From a practical application point of view, production level systems do not always have access to the full-text of the paper, so having the ability to generate a \tldr solely from the abstract would be useful.

% Therefore, for each baseline method, we consider two setups as the input: (1) the abstract only and (2) the abstract plus introduction and conclusion sections. We evaluate both extractive and abstractive baseline models. %Further, since there could be multiple valid \tldrs for each paper as discussed in \$[ADD REFERENCE TO SECTION THAT HAS THIS ANALYSIS], we present two sets of results: results that consider only the author written \tldrs as well as results that include both author \tldrs and worker rewritten \tldrs. 



==> tables/2-review_comment_example.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{@{}lr@{}}
    \toprule
    Reviewer comment & \begin{tabular}[c]{@{}p{12cm}@{}}
    The authors proposed a new clustering algorithm named deep continuous clustering (DCC) that integrates autoencoder into continuous clustering. As a variant of continuous clustering (RCC), DCC formed a global continuous objective for joint nonlinear dimensionality reduction and clustering. The objective can be directly optimized using SGD like method. Extensive experiments on image and document datasets show the effectiveness of DCC. However, part of experiments are not comprehensive enough. The idea of integrating autoencoder with continuous clustering is novel, and the optimization part is quite different. The trick used in the paper (sampling edges but not samples) looks interesting and seems to be effective. In the following, there are some detailed comments: 1. The paper is well written and easy to follow, except the definition of Geman-McClure function is...
    \end{tabular} \\ \hdashline[0.4pt/2pt]
    Peer Review \tldr & \begin{tabular}[c]{@{}p{12cm}@{}} Deep Continuous Clustering is a clustering method that integrates the autoencoder objective with the clustering objective then train using SGD. \end{tabular} \\ 
    \hdashline[0.4pt/2pt]
    Author-\tldr & \begin{tabular}[c]{@{}p{12cm}@{}} A clustering algorithm that performs joint nonlinear dimensionality reduction and clustering by optimizing a global continuous objective. \end{tabular} \\\bottomrule
    \end{tabular}
    \caption{Example of a reviewer's comment rewritten as a \tldr}
    \label{tab:review-comment-example}
    \end{table*}

==> tables/abstractive-results.tex <==
% \begin{table*}[]
% \centering
% \begin{tabular}{l|lll|lll}
%  & \multicolumn{3}{c|}{\textbf{\dataset-A}} & \multicolumn{3}{c}{\textbf{\dataset-AIC}} \\ \hline
% \textbf{Method} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} \\ \hline
% \textbf{GPT2 + dataset} & 23.5 & 6.2 & 19.9 & -1 & -1 & -1 \\ \hline
% \textbf{BART.LARGE} & 22.6 & 7.2 & 19.6 & -1 & -1 & -1 \\ \hline
% \textbf{BART.LARGE.XSUM} & 26.2 & 9.2 & 22.3 & 22.6 & 7.2 & 19.6 \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}BART.LARGE +\\ \dataset\end{tabular}} & 34.2 & 16.3 & 30.3 & 27.4 & 10.2 & 23.2 \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}BART.LARGE.XSUM\\ + \dataset\end{tabular}} & 33.8 & 15.8 & 29.8 & 32.6 & 14.4 & 28.4
% \end{tabular}
% \label{abstractive-results}
% \caption{Results on abstractive baselines}
% \end{table*}

% \begin{table*}[]
% \centering
% \small
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
%  & \multicolumn{3}{c}{\textbf{\dataset-A}} & \multicolumn{3}{c}{\textbf{\dataset-AIC}} \\ 
%  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% \textbf{Method} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} \\ \midrule
% \textbf{GPT2 + dataset} & 23.5 & 6.2 & 19.9 & -1 & -1 & -1 \\ 
% BART-large & 22.6 & 7.2 & 19.6 & -1 & -1 & -1 \\ 
% BART-large + XSUM & 26.2 & 9.2 & 22.3 & 22.6 & 7.2 & 19.6 \\ 
% \begin{tabular}[c]{@{}l@{}}BART-large +\\ \dataset\end{tabular} & 34.2 & 16.3 & 30.3 & 27.4 & 10.2 & 23.2 \\ 
% \begin{tabular}[c]{@{}l@{}}BART-large + XSUM\\ + \dataset\end{tabular} & 33.8 & 15.8 & 29.8 & 32.6 & 14.4 & 28.4\\ \bottomrule
% \end{tabular}
% \label{abstractive-results}
% \caption{Results on abstractive baselines}
% \end{table*}
\setlength\dashlinedash{0.2pt}
\setlength\dashlinegap{1.5pt}
\setlength\arrayrulewidth{0.3pt}


\begin{table*}
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
   & \multicolumn{3}{c}{\textbf{\ao}} & \multicolumn{3}{c}{\textbf{\aic}} \\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7}
\textbf{Method}   & Rouge-1 & Rouge-2 & Rouge-L & Rouge-1 & Rouge-2 & Rouge-L \\ \midrule
\textit{Ext. Oracle}  & 47.7 & 24.7 & 38.5 & 52.4 & 29.0 & 42.9 \\ \cdashline{1-7}
% \textit{Ext. baselines} & & & & & & \\
% \hspace{1em}Title Heuristic & 36.7 & 15.7 & 28.8 & 36.5 & 14.9 & 28.5 \\
PACSUM \cite{Zheng2019PACSUM} & 22.5 & 7.5 & 17.4 & 23.0	& 7.4 & 17.8 \\ 
%\textbf{Unsupervised + SCIBERT} & 0.228 & 0.074 & 0.176 & 0.229 & 0.075 & 0.177 \\ \hline
%\textbf{Unsupervised + ROBERTA} & 0.229 & 0.074 & 0.177 & 0.230 & 0.074 & 0.178 \\ \hline
BERTSUMEXT \cite{Liu2019TextSW} & 36.7	& 15.8 & 29.4 & 28.3 & 10.4 & 23.5\\ \cdashline{1-7}
%  \textit{Abst. baselines} & & & & & & \\
%  \hspace{1em}GPT2 + \dataset & 22.8 & 7.5 & 17.4 & -1 & -1 & -1 \\ 
% BART-large \cite{Lewis2019BARTDS} & 30.1 & 10.2 & 22.6 & 28.9 & 9.3 & 21.9 \\ 
% BART-large + XSUM & 34.4 & 12.3 & 27.0 & 35.9	& 13.6	& 28.2 \\ 
\begin{tabular}[c]{@{}l@{}}BART-large + \dataset\end{tabular} \cite{Lewis2019BARTDS} & 41.6 & 19.8 & 33.8 & 42.0	& 20.5	& 34.9 \\ 
% \begin{tabular}[c]{@{}l@{}}BART-large + XSUM + \dataset  \end{tabular} & 41.2	 & 19.7	& 33.4 & 43.2 & \textbf{21.2} & 35.6\\
\cdashline{1-7}
\begin{tabular}[c]{@{}l@{}}BART-large + XSUM + Multitask-CTRL (Title/\dataset)\end{tabular} & \textbf{42.6} &\textbf{ 21.0} & \textbf{34.8} & \textbf{43.4 }& 21.0 & \textbf{35.6}\\
%\hspace{1em}\begin{tabular}[c]{@{}l@{}}BART-large + XSUM + Title-Gen +  \dataset\end{tabular} & -1 & -1 & -1 & -1 & -1 & -1\\ 
\bottomrule
\end{tabular}
\caption{Main results of \tldr generation comparing our method with extractive and abstractive baselines. In \dataset-A the input is the abstract, while in \dataset-AIC the input to the models is abstract+introduction+conclusion sections.}\label{tab:results}
\end{table*}

==> tables/gold-variation.tex <==
\begin{table}[hbt!]
\centering
\small
\begin{tabular}{@{}lrrr@{}}
\toprule
\textit{Avg. Num Words} &  \\
\tldr-Auth & 18.9 \\
\tldr-PR & 22.9  \\
\midrule
\textit{Avg. Jaccard } &  \\
1-gram & 15.0  \\
2-gram & 2.5  \\
3-gram & 0.7  \\
\bottomrule
\end{tabular}
\caption{Metrics comparing \tldr-Auth and \tldr-PR}
\label{tab:gold-variation}
\end{table}

==> tables/main_results.tex <==
\setlength\dashlinedash{0.2pt}
\setlength\dashlinegap{1.5pt}
\setlength\arrayrulewidth{0.3pt}


\begin{table*}
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lrrr@{\hspace{2.8em}}rrr@{}}
\toprule
   & \multicolumn{3}{c}{\textbf{\ao}} & \multicolumn{3}{c}{\textbf{\aic}} \\ 
 \cmidrule(l{2pt}r{20pt}){2-4} \cmidrule(lr){5-7}
\textbf{Method}   & Rouge-1 & Rouge-2 & Rouge-L & Rouge-1 & Rouge-2 & Rouge-L \\ \midrule
\textit{Ext. Oracle}  & 47.7 & 24.7 & 38.5 & 52.4 & 29.0 & 42.9 \\ [0.5ex]
\hdashline\noalign{\vskip 0.5ex}
% \textit{Ext. baselines} & & & & & & \\
% \hspace{1em}Title Heuristic & 36.7 & 15.7 & 28.8 & 36.5 & 14.9 & 28.5 \\
PACSUM \cite{Zheng2019PACSUM} & 22.5 & 7.5 & 17.4 & 23.0	& 7.4 & 17.8 \\ 
%\textbf{Unsupervised + SCIBERT} & 0.228 & 0.074 & 0.176 & 0.229 & 0.075 & 0.177 \\ \hline
%\textbf{Unsupervised + ROBERTA} & 0.229 & 0.074 & 0.177 & 0.230 & 0.074 & 0.178 \\ \hline
BERTSUMEXT \cite{Liu2019TextSW} & 36.7	& 15.8 & 29.4 & 28.3 & 10.4 & 23.5\\ [0.5ex]
\hdashline\noalign{\vskip 0.5ex}
%  \textit{Abst. baselines} & & & & & & \\
%  \hspace{1em}GPT2 + \dataset & 22.8 & 7.5 & 17.4 & -1 & -1 & -1 \\ 
% BART-large \cite{Lewis2019BARTDS} & 30.1 & 10.2 & 22.6 & 28.9 & 9.3 & 21.9 \\ 
% BART-large + XSUM & 34.4 & 12.3 & 27.0 & 35.9	& 13.6	& 28.2 \\ 
\begin{tabular}[c]{@{}l@{}}T5 \end{tabular} \cite{T5-Raffel2019ExploringTL} \todoit{complete} & 0.1 & 0.1 & 0.1 & 0.1	& 0.1	& 0.1 \\ 
\begin{tabular}[c]{@{}l@{}}T5.XSUM \cite{T5-Raffel2019ExploringTL} \todoit{complete} \end{tabular} & 0.2	 & 0.2	& 0.2 & 0.2 & 0.2 & 0.2\\ [0.5ex]
\begin{tabular}[c]{@{}l@{}}BART \end{tabular} \cite{Lewis2019BARTDS} & 42.5 & 20.8 & 35.0 & 42.0	& 20.5	& 34.9 \\ 
\begin{tabular}[c]{@{}l@{}}BART.XSUM \cite{Lewis2019BARTDS} \end{tabular} & 42.5	 & 21.1	& 34.9 & 43.2 & \textbf{21.2} & 35.6\\ [0.5ex]
\hdashline\noalign{\vskip 0.5ex}
\begin{tabular}[c]{@{}l@{}}\ours$_{T5}$ (Ours) \todoit{complete}\end{tabular} & \textbf{42.6} &\textbf{ 21.0} & \textbf{34.8} & \textbf{43.4 }& 21.0 & \textbf{35.6}\\
\begin{tabular}[c]{@{}l@{}}\ours$_{BART}$ (Ours)\end{tabular} & \textbf{44.2} &\textbf{21.1} & \textbf{35.8} & \textbf{43.4 }& 21.0 & \textbf{35.6}
\\
%\hspace{1em}\begin{tabular}[c]{@{}l@{}}BART-large + XSUM + Title-Gen +  \dataset\end{tabular} & -1 & -1 & -1 & -1 & -1 & -1\\ 
\bottomrule
\end{tabular}
\caption{Main results of \tldr generation comparing our method with extractive and abstractive baselines. In \ao the input is the abstract, while in \aic the input to the models is abstract+introduction+conclusion sections. All baselines are finetuned on \dataset, except for PACSUM, our unsupervised baseline.}\label{tab:results}
\end{table*}

==> tables/main_results2.tex <==
\setlength\dashlinedash{0.2pt}
\setlength\dashlinegap{1.5pt}
\setlength\arrayrulewidth{0.3pt}


\begin{table*}
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lrrr@{\hspace{2.8em}}rrr@{}}
\toprule
   & \multicolumn{3}{c}{\textbf{\ao}} & \multicolumn{3}{c}{\textbf{\aic}} \\ 
 \cmidrule(l{2pt}r{20pt}){2-4} \cmidrule(lr){5-7}
\textbf{Method}   & Rouge-1 & Rouge-2 & Rouge-L & Rouge-1 & Rouge-2 & Rouge-L \\ \midrule
\textit{Ext. Oracle}  & 47.7 & 24.7 & 38.5 & 52.4 & 29.0 & 42.9 \\ [0.5ex]
\hdashline\noalign{\vskip 0.5ex}
% \textit{Ext. baselines} & & & & & & \\
% \hspace{1em}Title Heuristic & 36.7 & 15.7 & 28.8 & 36.5 & 14.9 & 28.5 \\
PACSUM \cite{Zheng2019PACSUM} & 22.5 & 7.5 & 17.4 & 23.0	& 7.4 & 17.8 \\ 
%\textbf{Unsupervised + SCIBERT} & 0.228 & 0.074 & 0.176 & 0.229 & 0.075 & 0.177 \\ \hline
%\textbf{Unsupervised + ROBERTA} & 0.229 & 0.074 & 0.177 & 0.230 & 0.074 & 0.178 \\ \hline
BERTSUMEXT \cite{Liu2019TextSW} & 36.7	& 15.8 & 29.4 & 28.3 & 10.4 & 23.5\\ [0.5ex]
\hdashline\noalign{\vskip 0.5ex}
%  \textit{Abst. baselines} & & & & & & \\
%  \hspace{1em}GPT2 + \dataset & 22.8 & 7.5 & 17.4 & -1 & -1 & -1 \\ 
% BART-large \cite{Lewis2019BARTDS} & 30.1 & 10.2 & 22.6 & 28.9 & 9.3 & 21.9 \\ 
% BART-large + XSUM & 34.4 & 12.3 & 27.0 & 35.9	& 13.6	& 28.2 \\ 
\begin{tabular}[c]{@{}l@{}}BART \end{tabular} \cite{Lewis2019BARTDS} & 41.6 & 19.8 & 33.8 & 42.0	& 20.5	& 34.9 \\ 
\begin{tabular}[c]{@{}l@{}}BART.XSUM \cite{Lewis2019BARTDS} \end{tabular} & 41.2	 & 19.7	& 33.4 & 43.2 & \textbf{21.2} & 35.6\\ [0.5ex]
\hdashline\noalign{\vskip 0.5ex}
\begin{tabular}[c]{@{}l@{}}\ours (Ours)\end{tabular} & \textbf{42.6} &\textbf{ 21.0} & \textbf{34.8} & \textbf{43.4 }& 21.0 & \textbf{35.6}\\
%\hspace{1em}\begin{tabular}[c]{@{}l@{}}BART-large + XSUM + Title-Gen +  \dataset\end{tabular} & -1 & -1 & -1 & -1 & -1 & -1\\ 
\bottomrule
\end{tabular}
\caption{Main results of \tldr generation comparing our method with extractive and abstractive baselines. In \ao the input is the abstract, while in \aic the input to the models is abstract+introduction+conclusion sections. All baselines are finetuned on \dataset, except for PACSUM, our unsupervised baseline.}\label{tab:results}
\end{table*}

==> tables/n-gram-overlap.tex <==
\begin{table}[hbt!]
\centering
\small
\begin{tabular}{@{}lrrr@{}}
\toprule
 & 1-gram & 2-gram & 3-gram \\ \midrule
XSUM & 35.8 & 83.5 & 95.5 \\
CNN & 16.8 & 54.3 & 72.4 \\
DailyMail & 17.0 & 53.8 & 72.1 \\
Newsroom & 26.0 &  52.3 &  61.3 \\
Arxiv & 8.3  &  40.8 &  67.2 \\
PigPatent & 13.6 & 53.0 & 78.8 \\
SciSummNet & 7.4 &   23.7 &  31.7 \\
CLPubSum  & 7.7 &    41.9 &  71.6 \\
[0.5ex]
\hdashline[0.5pt/0.5pt]\noalign{\vskip 0.5ex}
\dataset & 10.76  &  45.92 &  69.35  \\
% \hspace{1ex} \tldr-Auth & - & - & - \\
% \hspace{1ex} \tldr-PR & - & - & - \\
% \hspace{1ex} \ao & 25.99 & 65.75 & 79.62 \\
% \hspace{1ex} \aic & 11.30 & 47.60 & 68.54 \\
% \hspace{1ex} $\mathrm{\dataset_{Full}}$ & 5.65 & 21.57 & 62.60 \\    

% \multicolumn{1}{r}{\textbf{-Full-Text}} & 5.65 & 21.57 & 62.60 \\
% \textbf{\dataset-A} & 25.99 & 65.75 & 79.62 \\
% \multicolumn{1}{r}{\textbf{-AIC}} & 11.30 & 47.60 & 68.54 \\
% \multicolumn{1}{r}{\textbf{-Full-Text}} & 5.65 & 21.57 & 62.60 \\ 
\bottomrule
\end{tabular}
\caption{Percentage of n-grams in summary that are not in source document (i.e., novelty).
% For \dataset we show analysis of different sections as the source document.
}
\label{tab:n-gram-overlap}
\end{table}

==> tables/other-experiements.tex <==
% \begin{table*}[]
% \centering
% \begin{tabular}{l|lll|lll}
%  & \multicolumn{3}{c|}{\textbf{\dataset-A}} & \multicolumn{3}{c}{\textbf{\dataset-AIC}} \\ \hline
% \textbf{Method} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} \\ \hline
% \textbf{GPT2 + dataset} & 23.5 & 6.2 & 19.9 & -1 & -1 & -1 \\ \hline
% \textbf{BART.LARGE} & 22.6 & 7.2 & 19.6 & -1 & -1 & -1 \\ \hline
% \textbf{BART.LARGE.XSUM} & 26.2 & 9.2 & 22.3 & 22.6 & 7.2 & 19.6 \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}BART.LARGE +\\ \dataset\end{tabular}} & 34.2 & 16.3 & 30.3 & 27.4 & 10.2 & 23.2 \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}BART.LARGE.XSUM\\ + \dataset\end{tabular}} & 33.8 & 15.8 & 29.8 & 32.6 & 14.4 & 28.4
% \end{tabular}
% \label{abstractive-results}
% \caption{Results on abstractive baselines}
% \end{table*}

% \begin{table*}[]
% \centering
% \small
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
%  & \multicolumn{3}{c}{\textbf{\dataset-A}} & \multicolumn{3}{c}{\textbf{\dataset-AIC}} \\ 
%  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% \textbf{Method} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} \\ \midrule
% \textbf{GPT2 + dataset} & 23.5 & 6.2 & 19.9 & -1 & -1 & -1 \\ 
% BART-large & 22.6 & 7.2 & 19.6 & -1 & -1 & -1 \\ 
% BART-large + XSUM & 26.2 & 9.2 & 22.3 & 22.6 & 7.2 & 19.6 \\ 
% \begin{tabular}[c]{@{}l@{}}BART-large +\\ \dataset\end{tabular} & 34.2 & 16.3 & 30.3 & 27.4 & 10.2 & 23.2 \\ 
% \begin{tabular}[c]{@{}l@{}}BART-large + XSUM\\ + \dataset\end{tabular} & 33.8 & 15.8 & 29.8 & 32.6 & 14.4 & 28.4\\ \bottomrule
% \end{tabular}
% \label{abstractive-results}
% \caption{Results on abstractive baselines}
% \end{table*}
\setlength\dashlinedash{0.2pt}
\setlength\dashlinegap{1.5pt}
\setlength\arrayrulewidth{0.3pt}


\begin{table*}[hbt!]
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lrrr@{\hspace{2.8em}}rrr@{}}
\toprule
   & \multicolumn{3}{c}{\textbf{\ao}} & \multicolumn{3}{c}{\textbf{\aic}} \\ 
 \cmidrule(l{2pt}r{20pt}){2-4} \cmidrule(lr){5-7}
\textbf{Method}   & Rouge-1 & Rouge-2 & Rouge-L & Rouge-1 & Rouge-2 & Rouge-L \\ \midrule
\begin{tabular}[c]{@{}l@{}} BART.XSUM $\to$ \dataset \end{tabular} & 41.2	 & 19.7	& 33.4 & 43.2 & \textbf{21.2} & 35.6\\
\cdashline{1-7}
% BART-large (no \tldr finetuning) & 30.1 & 10.2 & 22.6 & 28.9 & 9.3 & 21.9 \\ 
% BART-large + XSUM (no \tldr finetuning) & 34.4 & 12.3 & 27.0 & 35.9	& 13.6	& 28.2 \\ 
\hspace{1.78cm}  $\to$ arXiv titles $\to$ \dataset & 17.7 & 2.7 & 13.9 & 21.9 & 2.2 & 17.8 \\
\hspace{1.78cm} $\to$ arXiv titles + \dataset (no codes) & 40.5 & 19.5 & 33.5 & 42.6 &	21.0 & 34.8 \\
\begin{tabular}[c]{@{}l@{}} \hspace{1.78cm} $\to$ Title + \dataset (with codes) \end{tabular} & \textbf{42.6} &\textbf{ 21.0} & \textbf{34.8} & \textbf{43.4 }& 21.0 & \textbf{35.6}\\
\bottomrule
\end{tabular}
\caption{Alternative training configurations. Arrows ``$\to$'' indicate finetuning.  Plus signs ``+'' indicate multitask training with shuffled data.  The final model is \ours. \kyle{This table is kinda bad; we might not even need it; just create mini paragraphs to answer each question in text} }\label{tab:other-results}
\end{table*}

==> tables/title-gen-results.tex <==
% \begin{table*}[]
% \centering
% \begin{tabular}{l|lll|lll}
%  & \multicolumn{3}{c|}{\textbf{\dataset-A}} & \multicolumn{3}{c}{\textbf{\dataset-AIC}} \\ \hline
% \textbf{Method} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} \\ \hline
% \textbf{GPT2 + dataset} & 23.5 & 6.2 & 19.9 & -1 & -1 & -1 \\ \hline
% \textbf{BART.LARGE} & 22.6 & 7.2 & 19.6 & -1 & -1 & -1 \\ \hline
% \textbf{BART.LARGE.XSUM} & 26.2 & 9.2 & 22.3 & 22.6 & 7.2 & 19.6 \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}BART.LARGE +\\ \dataset\end{tabular}} & 34.2 & 16.3 & 30.3 & 27.4 & 10.2 & 23.2 \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}BART.LARGE.XSUM\\ + \dataset\end{tabular}} & 33.8 & 15.8 & 29.8 & 32.6 & 14.4 & 28.4
% \end{tabular}
% \label{abstractive-results}
% \caption{Results on abstractive baselines}
% \end{table*}

% \begin{table*}[]
% \centering
% \small
% \begin{tabular}{@{}lrrrrrr@{}}
% \toprule
%  & \multicolumn{3}{c}{\textbf{\dataset-A}} & \multicolumn{3}{c}{\textbf{\dataset-AIC}} \\ 
%  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% \textbf{Method} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} \\ \midrule
% \textbf{GPT2 + dataset} & 23.5 & 6.2 & 19.9 & -1 & -1 & -1 \\ 
% BART-large & 22.6 & 7.2 & 19.6 & -1 & -1 & -1 \\ 
% BART-large + XSUM & 26.2 & 9.2 & 22.3 & 22.6 & 7.2 & 19.6 \\ 
% \begin{tabular}[c]{@{}l@{}}BART-large +\\ \dataset\end{tabular} & 34.2 & 16.3 & 30.3 & 27.4 & 10.2 & 23.2 \\ 
% \begin{tabular}[c]{@{}l@{}}BART-large + XSUM\\ + \dataset\end{tabular} & 33.8 & 15.8 & 29.8 & 32.6 & 14.4 & 28.4\\ \bottomrule
% \end{tabular}
% \label{abstractive-results}
% \caption{Results on abstractive baselines}
% \end{table*}
\setlength\dashlinedash{0.2pt}
\setlength\dashlinegap{1.5pt}
\setlength\arrayrulewidth{0.3pt}


\begin{table*}
\centering
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
   & \multicolumn{3}{c}{\textbf{\ao}} & \multicolumn{3}{c}{\textbf{\aic}} \\ 
 \cmidrule(lr){2-4} \cmidrule(lr){5-7}
\textbf{Method}   & Rouge-1 & Rouge-2 & Rouge-L & Rouge-1 & Rouge-2 & Rouge-L \\ \midrule
\textit{Ext. Oracle}  & 47.7 & 24.7 & 38.5 & 52.4 & 29.0 & 42.9 \\ \cdashline{1-7}
% \textit{Ext. baselines} & & & & & & \\
% \hspace{1em}Title Heuristic & 36.7 & 15.7 & 28.8 & 36.5 & 14.9 & 28.5 \\
PACSUM \cite{Zheng2019PACSUM} & 22.5 & 7.5 & 17.4 & 23.0	& 7.4 & 17.8 \\ 
%\textbf{Unsupervised + SCIBERT} & 0.228 & 0.074 & 0.176 & 0.229 & 0.075 & 0.177 \\ \hline
%\textbf{Unsupervised + ROBERTA} & 0.229 & 0.074 & 0.177 & 0.230 & 0.074 & 0.178 \\ \hline
BERTSUMEXT \cite{Liu2019TextSW} & 36.7	& 15.8 & 29.4 & 28.3 & 10.4 & 23.5\\ \cdashline{1-7}
%  \textit{Abst. baselines} & & & & & & \\
%  \hspace{1em}GPT2 + \dataset & 22.8 & 7.5 & 17.4 & -1 & -1 & -1 \\ 
BART-large \cite{Lewis2019BARTDS} & 30.1 & 10.2 & 22.6 & 28.9 & 9.3 & 21.9 \\ 
BART-large + XSUM & 34.4 & 12.3 & 27.0 & 35.9	& 13.6	& 28.2 \\
\begin{tabular}[c]{@{}l@{}}BART-large + \dataset\end{tabular} & 41.6 & 19.8 & 33.8 & 42.0	& 20.5	& 34.9 \\ \cdashline{1-7}
\textit{This work} & & & & & & \\
\begin{tabular}[c]{@{}l@{}}BART-large + XSUM + \dataset  \end{tabular} & 41.2	 & 19.7	& 33.4 & 43.2 & \textbf{21.2} & 35.6\\
\begin{tabular}[c]{@{}l@{}}BART-large + XSUM + Multitask (Title/\dataset)\end{tabular} & \textbf{42.6} &\textbf{ 21.0} & \textbf{34.8} & \textbf{43.4 }& 21.0 & \textbf{35.6}\\
%\hspace{1em}\begin{tabular}[c]{@{}l@{}}BART-large + XSUM + Title-Gen +  \dataset\end{tabular} & -1 & -1 & -1 & -1 & -1 & -1\\ 
\bottomrule
\end{tabular}
\caption{Main results of \tldr generation comparing our method with extractive and abstractive baselines. In \dataset-A the input is the abstract, while in \dataset-AIC the input to the models is abstract+introduction+conclusion sections.}\label{tab:results}
\end{table*}

==> weld-defns.tex <==

\newcommand{\Comment}[1]{} 
\newcommand{\NOTE}[1]{\marginpar{\em {#1}}}
\newcommand{\bug}
    {\mbox{\rule{2mm}{2mm}}}
\newcommand{\Bug}[1]
    {\bug \footnote{BUG: {#1}}}
\newcommand{\QED}{\mbox{$\Box$}}
\newcommand{\ddt}{\mbox{$\frac{d}{dt}\,$}}  %* no strut

\newcommand{\etal}{\mbox{\it et al.}}
\newcommand{\etc}{\mbox{\it etc.}}
\newcommand{\eg}{\mbox{\it e.g.}}
\newcommand{\ie}{\mbox{\it i.e.}}
\newcommand{\cf}{\mbox{\it cf.}}
\newcommand{\Eg}{\mbox{\it E.g.}}
\newcommand{\Ie}{\mbox{\it I.e.}}
\newcommand{\?}{\mbox{?}}




\newcommand{\DEFN}{\mbox{$\stackrel{\mbox{\tiny def}}{=}$}}

\newcommand{\TT}[1]{\mbox{\tt #1}}
%\newcommand{\bi}{\begin{itemize}}
%\newcommand{\ei}{\end{itemize}}
\newcommand{\bi}{\begin{list}{$\bullet$}{
    \setlength{\leftmargin}{1.5 em}
    \setlength{\itemsep}{0 pt}
    \setlength{\topsep}{3 pt}
    \setlength{\parsep}{3 pt}
    \setlength{\partopsep}{0 pt}
    \setlength{\labelwidth}{1 em}
    \setlength{\labelsep}{0.5 em}
    \setlength{\parskip}{0cm}  }}
\newcommand{\ei}{\end{list}}

\newcommand{\BE}{\begin{enumerate}}
\newcommand{\EE}{\end{enumerate}}

%\newtheorem{defnctr}{Definition}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}        
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{propos}[theorem]{Proposition}
%\newcommand{\proof}
%	{\vspace{-8pt}
%	 {\bf Proof:}}



\newcommand{\tuple}[1]
        {\mbox{$\langle{#1}\rangle$}}
\newcommand{\set}[1]
        {\mbox{$\{{#1}\}$}}
\newcommand{\size}[1]{\mbox{$\mid\!#1\!\mid$}}



\newcommand{\PROOF}[1]{\mbox{\noindent \proofbegin {#1} \proofend}}
\newcommand{\proofbegin}{\mbox{\bf Proof: \ }}
\newcommand{\proofend}{\Math{\Box}}
\newcommand{\st}{\mbox{ such that }}
\newcommand{\wht}{\mbox{ we have that }}
\newcommand{\entails}{\mbox{$\models$}}
\newcommand{\yields}{\mbox{$\models$}}
\newcommand{\dgets}{\mbox{$\leftarrow$}}

%\renewcommand{\baselinestretch}{0.985}




\newcommand{\initab}{                           % set up tab stops
\begin{tabbing}
XXX \= XXXX \= \kill
}
\newcommand{\begpub}{
\begin{quotation}
\noindent
}
\newcommand{\nextpub}{

\vspace{2mm}
\noindent
}
\newcommand{\finpub}{
\end{quotation}
}



\hyphenation{non-de-ter-mi-nis-tic-al-ly non-de-ter-mi-nis-tic
exis-ten-tial-ly quan-tified se-lec-tion exis-ting in-stan-tiated
uni-vers-al-ly es-tab-lish in-con-sis-tent}


% \newcommand{\ncd}{\mbox{$\neq$}}
% \newcommand{\cd}{\mbox{$=$}}
% \newcommand{\fabian}{\mbox{\sc fabian}}
% \newcommand{\occam}{\mbox{\sc occam}}
% \newcommand{\sadl}{\mbox{\sc sadl}}
% \newcommand{\socrates}{\mbox{\sc socrates}}
% \newcommand{\uwl}{\mbox{\sc uwl}}
% \newcommand{\spa}{\mbox{\sc spa}}
% \newcommand{\scr}{\mbox{\sc scr}}
% \newcommand{\strips}{\mbox{\sc strips}}
% \newcommand{\snlp}{\mbox{\sc snlp}}
% \newcommand{\cbur}{\mbox{\sc C-buridan}}
% \newcommand{\buridan}{\mbox{\sc buridan}}
% \newcommand{\xii}{\mbox{\sc xii}}
% \newcommand{\zeno}{\mbox{\sc zeno}}
% \newcommand{\adl}{\mbox{\sc adl}}
% \newcommand{\kr}{\mbox{\tt /kr94}}
% \newcommand{\ucpop}{\mbox{\sc ucpop}}
% 
% \newcommand{\cause}{{\tt cause}}
% \newcommand{\observe}{{\tt observe}}
% \newcommand{\satisfy}{{\tt satisfy}}
% \newcommand{\handsoff}{{\tt hands-off}}
% \newcommand{\findout}{{\tt find-out}}
% 
% \newcommand{\CAUS}{\mbox{C}}
% \newcommand{\OBS}{\mbox{O}}
% \newcommand{\PAT}{\mbox{\sf E}}
% \newcommand{\fact}{\mbox{$\varphi$}}
% \newcommand{\LIT}{\mbox{\sf p}}
% \newcommand{\lit}{\mbox{\LIT}}
% \newcommand{\litp}{\mbox{\LIT$^\prime$}}
% \newcommand{\rel}{\mbox{REL}}
% \newcommand{\change}[3]{\mbox{$\Delta(#1,{\tt #2}\rightarrow {\tt #3})$}}   
% 
% \newcommand{\true}{{\tt T}}
% \newcommand{\false}{{\tt F}}
% \newcommand{\unknown}{{\tt U}}
% 
%

 
